A comparative study of scalable multilevel preconditioners for cardiac mechanics

In this work, we provide a performance comparison between the Balancing Domain Decomposition by Constraints (BDDC) and the Algebraic Multigrid (AMG) preconditioners for cardiac mechanics on both structured and unstructured finite element meshes. The mechanical behavior of myocardium can be described by the equations of three-dimensional finite elasticity, which are discretized by finite elements in space and yield the solution of a large scale nonlinear algebraic system. This problem is solved by a Newton-Krylov method, where the solution of the Jacobian linear system is accelerated by BDDC/AMG preconditioners. We thoroughly explore the main parameters of the BDDC preconditioner in order to make the comparison fair. We focus on: the performance of different direct solvers for the local and coarse problems of the BDDC algorithm; the impact of the different choices of BDDC primal degrees of freedom; and the influence of the finite element degree. Scalability tests are performed on Linux clusters up to 1024 processors, and we conclude with a performance study on a realistic electromechanical simulation.

==> tikz/EM/large-p2.tex <==
    \newcommand{\tagcolor}{yellow!20!white}
    \newcommand{\tzero}{0}
    \newcommand{\ttagone}{0.075}
    \newcommand{\tone}{0.13}
    \newcommand{\ttagtwo}{0.23}
    \newcommand{\ttwo}{0.31}
    \newcommand{\ttagthree}{0.42}
    \newcommand{\tthree}{0.475}
    \newcommand{\ttagfour}{0.57}
    \newcommand{\tfour}{0.80}
    \newcommand{\ytag}{700}
    \newcommand{\ytop}{1000}
    \newcommand{\timetag}{240}
    \newcommand{\timetop}{320}
    \centering
    \begin{subfigure}{\textwidth}
    \begin{plot}[height=7cm, legend pos=north east,  legend style={at={(0.9, 0.9)}, anchor=north east}]{Time}{Average linear its.}
        \addplot+[fill opacity=0.1, mark=none] table [x=time, y=mechanics_iterations_linear_avg, col sep=comma, select coords between index={2}{160}] {data/EM/electromechanics-sr-p2.csv};
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_iterations_linear_avg, col sep=comma] {data/EM/electromechanics-sr-bddc-p2.csv};
        % Isovolumic contraction
        \addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tzero,0) (\tone,0) (\tone,\ytop) (0,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagone,\ytag) {\small IC};
		% Contraction 
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tone,0) (\ttwo,0) (\ttwo,\ytop) (\tone,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagtwo,\ytag) {\small C};
		% Isovol relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\ttwo,0) (\tthree,0) (\tthree,\ytop) (\ttwo,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagthree,\ytag) {\small IR};
		% Relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tthree,0) (\tfour,0) (\tfour,\ytop) (\tthree,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagfour,\ytag) {\small R};
        \legend{AMG, BDDC}
    \end{plot}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \begin{plot}[height=7cm,  legend style={at={(0.9, 0.9)}, anchor=north east}]{Time}{Solution time}
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_solving_time, col sep=comma] {data/EM/electromechanics-sr-p2.csv};
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_solving_time, col sep=comma] {data/EM/electromechanics-sr-bddc-p2.csv};
        % Isovolumic contraction
        \addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tzero,0) (\tone,0) (\tone,\timetop) (0,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagone,\timetag) {\small IC};
		% Contraction 
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tone,0) (\ttwo,0) (\ttwo,\timetop) (\tone,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagtwo,\timetag) {\small C};
		% Isovol relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\ttwo,0) (\tthree,0) (\tthree,\timetop) (\ttwo,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagthree,\timetag) {\small IR};
		% Relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tthree,0) (\tfour,0) (\tfour,\timetop) (\tthree,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagfour,\timetag) {\small R};
        \legend{AMG, BDDC}
    \end{plot}
    \end{subfigure}

==> tikz/EM/small-p2.tex <==
    \newcommand{\tagcolor}{yellow!20!white}
    \newcommand{\tzero}{0}
    \newcommand{\ttagone}{0.075}
    \newcommand{\tone}{0.13}
    \newcommand{\ttagtwo}{0.23}
    \newcommand{\ttwo}{0.31}
    \newcommand{\ttagthree}{0.42}
    \newcommand{\tthree}{0.475}
    \newcommand{\ttagfour}{0.57}
    \newcommand{\tfour}{0.50}
    \newcommand{\ytag}{700}
    \newcommand{\ytop}{1000}
    \newcommand{\timetag}{500}
    \newcommand{\timetop}{620}
    \centering
    \begin{subfigure}{\textwidth}
    \begin{plot}[height=7cm, legend pos=north east,  legend style={at={(0.9, 0.9)}, anchor=north east}]{Time}{Average linear its.}
        \addplot+[fill opacity=0.1, mark=none] table [x=time, y=mechanics_iterations_linear_avg, col sep=comma, select coords between index={2}{160}] {data/EM/electromechanics-sr-p2-small.csv};
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_iterations_linear_avg, col sep=comma] {data/EM/electromechanics-sr-bddc-p2-small.csv};
        % Isovolumic contraction
        \addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tzero,0) (\tone,0) (\tone,\ytop) (0,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagone,\ytag) {\small IC};
		% Contraction 
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tone,0) (\ttwo,0) (\ttwo,\ytop) (\tone,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagtwo,\ytag) {\small C};
		% Isovol relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\ttwo,0) (\tthree,0) (\tthree,\ytop) (\ttwo,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagthree,\ytag) {\small IR};
		% Relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tthree,0) (\tfour,0) (\tfour,\ytop) (\tthree,\ytop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagfour,\ytag) {\small R};
        \legend{AMG, BDDC}
    \end{plot}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \begin{plot}[height=7cm,  legend style={at={(0.9, 0.9)}, anchor=north east}]{Time}{Solution time}
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_solving_time, col sep=comma] {data/EM/electromechanics-sr-p2-small.csv};
        \addplot+[fill opacity=0.1, mark=none, select coords between index={2}{160}] table [x=time, y=mechanics_solving_time, col sep=comma] {data/EM/electromechanics-sr-bddc-p2-small.csv};
        % Isovolumic contraction
        \addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tzero,0) (\tone,0) (\tone,\timetop) (0,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagone,\timetag) {\small IC};
		% Contraction 
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tone,0) (\ttwo,0) (\ttwo,\timetop) (\tone,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagtwo,\timetag) {\small C};
		% Isovol relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\ttwo,0) (\tthree,0) (\tthree,\timetop) (\ttwo,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagthree,\timetag) {\small IR};
		% Relaxation
		\addplot+[fill, mark=none, opacity=0.1] coordinates 
		{(\tthree,0) (\tfour,0) (\tfour,\timetop) (\tthree,\timetop)} \closedcycle;
		\node[fill=\tagcolor, text centered] 
		at (\ttagfour,\timetag) {\small R};
        \legend{AMG, BDDC}
    \end{plot}
    \end{subfigure}

==> tikz/local_solver.tex <==
    \begin{tikzpicture}
    \begin{axis}
        [ybar,
        xtick=data,
        width=6cm,
        height=6cm,
        ymin=0,
        % ymax=4.5,
        % ytick=data,
        ylabel=Time (s),
        bar width=5pt,
        enlarge x limits={abs=20pt},  % This keeps columns centered
        symbolic x coords={Beam, Swelling, Realistic},
         legend style={at={(0.03,0.97)},anchor=north west, fill opacity=0.6, font=\small,legend cell align=left}
        ]
        % \addplot[draw = yellow,line width = .4mm,fill = red] coordinates             {(a,0) (b,1)};
        MKL
        \addplot coordinates {(Beam,359.094) 
                              (Swelling, 480.194)
                              (Realistic, 768.288)};
        % Mumps
        \addplot coordinates {(Beam,350.929) 
                              (Swelling,  469.810)
                              (Realistic, 743.524)};
        SuperLU
        \addplot coordinates {(Beam,5276.573)
                              (Swelling, 2158.610)
                              (Realistic,3367.100)};
        % PETSc
        \addplot coordinates {(Beam,1467.854)
                              (Swelling, 9545.070)
                              (Realistic, 14469.941)};
    \legend{MKL\_Pardiso, Mumps, SuperLU, PETSc }
    % \legend{Mumps, PETSc, SuperLU}
    \end{axis}
    \end{tikzpicture}

==> tikz/weak/weak_scaling_beam_iterations.tex <==
    \begin{tikzpicture}
    \begin{semilogxaxis}
        [width=\textwidth,
        % height=8cm,
        % ymin=0,
        % ymax=4.5,
        % ytick=data,
        xlabel=CPU Cores,
        ylabel=Average GMRES iterations,
        % bar width=5pt,
        % enlarge x limits={abs=20pt},  % This keeps columns centered
         legend style={fill opacity=0.6, font=\tiny,legend cell align=left}
        ]
        
        % beam Q1
        \addplot [color=green!90!black, mark=triangle] coordinates {
                                (2, 2.166666667)
                                (16, 28.66666667)
                                (128, 38)
                                (1024, 39.5)};
                                
        % beam Q2
        \addplot [color=green!30!black, mark=square] coordinates {
                                (2, 2.166666667)
                                (16, 28.91666667)
                                (128, 34.16666667)
                                (1024, 38.52777778)};

        
        % beam amg Q1
        \addplot [color=yellow!80!black, mark=triangle] coordinates {
                                (2, 25.5)
                                (16, 25.33333333)
                                (128, 26.83333333)
                                (1024, 24.5)};
        % beam amg Q2
        \addplot [color=yellow!30!black, mark=square] coordinates {
                                (2, 31)
                                (16, 33.11111111)
                                (128, 54)};
    \legend{beam Q1, beam Q2, beam-AMG Q1, beam-AMG Q2}
    \end{semilogxaxis}
    \end{tikzpicture}
    
% ===== beam
% ======== Degree: 1
% (2, 16.062)
% (16, 21.143)
% (128, 24.005)
% (1024, 46.657)
% ======== Degree: 2
% (2, 28.600)
% (16, 37.284)
% (128, 48.200)
% (1024, 79.343)

% ===== beam amg
% ======== Degree: 1
% (2, 16.178)
% (16, 19.581)
% (128, 26.989)
% (1024, 77.049)
% ======== Degree: 2
% (2, 31.240)
% (16, 42.164)
% (128, 77.225)
% (1024, 0.0)


% ====== swelling
% ======== Degree: 1
% ======== Degree: 2


% ====== contraction
% ======== Degree: 1
% ======== Degree: 2


==> tikz/weak/weak_scaling_beam_time.tex <==
    \begin{tikzpicture}
    \begin{semilogxaxis}
        [width=\textwidth,
        height=8cm,
        % ymin=0,
        % ymax=4.5,
        % ytick=data,
        xlabel=CPU Cores,
        ylabel=Time (s),
        % bar width=5pt,
        % enlarge x limits={abs=20pt},  % This keeps columns centered
         legend style={fill opacity=0.6, font=\tiny,legend cell align=left}
        ]
        
        % beam Q1
        \addplot [color=green!90!black, mark=triangle] coordinates {
                                (2, 16.062)
                                (16, 21.143)
                                (128, 24.005)
                                (1024, 46.657)};
                                
        % beam Q2
        \addplot [color=green!30!black, mark=square] coordinates {
                                (2, 28.600)
                                (16, 37.284)
                                (128, 48.200)
                                (1024, 79.343)};

        
        % beam amg Q1
        \addplot [color=yellow!80!black, mark=triangle] coordinates {
                                (2, 16.178)
                                (16, 19.581)
                                (128, 26.989)
                                (1024, 77.049)};
        % beam amg Q2
        \addplot [color=yellow!30!black, mark=square] coordinates {
                                (2, 31.240)
                                (16, 42.164)
                                (128, 77.225)};
    \legend{beam Q1, beam Q2, beam-AMG Q1, beam-AMG Q2}
    \end{semilogxaxis}
    \end{tikzpicture}
    
% ===== beam
% ======== Degree: 1
% (2, 16.062)
% (16, 21.143)
% (128, 24.005)
% (1024, 46.657)
% ======== Degree: 2
% (2, 28.600)
% (16, 37.284)
% (128, 48.200)
% (1024, 79.343)

% ===== beam amg
% ======== Degree: 1
% (2, 16.178)
% (16, 19.581)
% (128, 26.989)
% (1024, 77.049)
% ======== Degree: 2
% (2, 31.240)
% (16, 42.164)
% (128, 77.225)
% (1024, 0.0)


% ====== swelling
% ======== Degree: 1
% ======== Degree: 2


% ====== contraction
% ======== Degree: 1
% ======== Degree: 2


==> tikz/weak/weak_scaling_contraction_time.tex <==
    \begin{tikzpicture}
    \begin{semilogxaxis}
        [width=\textwidth,
        height=8cm,
        % ymin=0,
        % ymax=4.5,
        % ytick=data,
        xlabel=CPU Cores,
        ylabel=Time (s),
        % bar width=5pt,
        % enlarge x limits={abs=20pt},  % This keeps columns centered
         legend style={fill opacity=0.6, font=\tiny,legend cell align=left}
        ]
        
        % beam Q1
        \addplot [color=green!90!black, mark=triangle] coordinates {
                                (16, 41.559)
                                (128, 62.529)
                                (1024, 480.423)};
                                
        % beam Q2
        \addplot [color=green!30!black, mark=square] coordinates {
                                (16, 46.492)
                                (128, 75.569)
                                (1024, 614.065)};

        
        % beam amg Q1
        \addplot [color=yellow!80!black, mark=triangle] coordinates {
                                (16, 38.212)
                                (128, 234.531)
                                (1024, 205.975)};
        % beam amg Q2
        \addplot [color=yellow!30!black, mark=square] coordinates {
                                (16, 57.592)
                                (128, 279.409)
                                (1024, 159.882)};
    \legend{beam Q1, beam Q2, beam-AMG Q1, beam-AMG Q2}
    \end{semilogxaxis}
    \end{tikzpicture}
    


==> tikz/weak/weak_scaling_swelling_time.tex <==
    \begin{tikzpicture}
    \begin{semilogxaxis}
        [width=\textwidth,
        height=8cm,
        % ymin=0,
        % ymax=4.5,
        % ytick=data,
        xlabel=CPU Cores,
        ylabel=Time (s),
        % bar width=5pt,
        % enlarge x limits={abs=20pt},  % This keeps columns centered
         legend style={fill opacity=0.6, font=\tiny,legend cell align=left}
        ]
        
        % beam Q1
        \addplot [color=green!90!black, mark=triangle] coordinates {
                                (16, 30.364)
                                (128, 55.090)
                                (1024, 250.850)};
                                
        % beam Q2
        \addplot [color=green!30!black, mark=square] coordinates {
                                (16, 270.664)
                                (128, 67.015)
                                (1024, 42.030)};

        
        % beam amg Q1
        \addplot [color=yellow!80!black, mark=triangle] coordinates {
                                (16, 31.001)
                                (128, 53.366)
                                (1024, 205.975)};
        % beam amg Q2
        \addplot [color=yellow!30!black, mark=square] coordinates {
                                (16, 52.703)
                                (128, 79.770)
                                (1024, 141.450)};
    \legend{beam Q1, beam Q2, beam-AMG Q1, beam-AMG Q2}
    \end{semilogxaxis}
    \end{tikzpicture}
    

